Diverse Multiple Trajectory Prediction Using a Two-stage Prediction Network Trained with Lane Loss

Prior arts in the field of motion predictions for autonomous driving tend to focus on finding a trajectory that is close to the ground truth trajectory. Such problem formulations and approaches, however, frequently lead to loss of diversity and biased trajectory predictions. Therefore, they are unsuitable for real-world autonomous driving where diverse and road-dependent multimodal trajectory predictions are critical for safety. To this end, this study proposes a novel loss function, \textit{Lane Loss}, that ensures map-adaptive diversity and accommodates geometric constraints. A two-stage trajectory prediction architecture with a novel trajectory candidate proposal module, \textit{Trajectory Prediction Attention (TPA)}, is trained with Lane Loss encourages multiple trajectories to be diversely distributed, covering feasible maneuvers in a map-aware manner. Furthermore, considering that the existing trajectory performance metrics are focusing on evaluating the accuracy based on the ground truth future trajectory, a quantitative evaluation metric is also suggested to evaluate the diversity of predicted multiple trajectories. The experiments performed on the Argoverse dataset show that the proposed method significantly improves the diversity of the predicted trajectories without sacrificing the prediction accuracy.

==> Sections/1_introduction.tex <==
Forecasting the future trajectories of dynamic agents in a multi-agent environment is a fundamental task for mobile robotics such as autonomous driving. To take action preemptively for an uncertain future, future motion predictions of nearby agents are necessary. 
However, future motions of nearby agents are highly uncertain, meaning that the deterministic strategy cannot aptly predict their future (e.g., selecting a single trajectory with the most likelihood). 
For this reason, predictions that can cover a wide range of uncertain futures, even those less likely to occur, are required in order for the decision/planning module to guarantee safety at all times so that an autonomous agent can beware of it. 

\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth]{Figures/RA-L Figures_final 1.pdf}
\vspace{-5pt}
\caption{Importance of diverse predictions. Prediction results with a single ground truth biased toward going straight tend to have a similar distribution to a biased GT distribution. However, our loss term, which leverages map-based pseudo GT, can cover diverse prediction results.} 
\label{figure:1}
\vspace{-15pt}
\end{figure}

Although numerous  trajectory prediction models have been introduced \cite{cslstm, lee2017desire, LaneGCN}, developing a reliable prediction model capable of generating multiple trajectories with diverse maneuvers remains challenging due to several issues. 
First, there is only a single ground truth modality per scenario in the datasets. The lack of diverse ground truth data for a given scenario poses a fundamental problem for multiple-trajectory predictions. 
Second, most trajectory datasets have a severely imbalanced distribution in which the lane-keeping trajectory is highly dominant compared to other maneuvers such as lane changes/turns. 
For example, in the Argoverse motion forecasting dataset \cite{chang2019argoverse}, one of the largest trajectory datasets, more than 90 percent of target agents' maneuvers are going straight, as presented in Table \ref{table:data distribution}.
Such an imbalance in the distribution of datasets leads to biased prediction results. 
Third, a driving environment such as a road map plays a key role in motion predictions, but existing methods cannot sufficiently learn a road map because it is only used as one of the inputs and is not explicitly used for supervision.


Previous works \cite{MTP,zhao2020tnt,covernet} have proposed several multi-modal prediction models with decent prediction accuracy in terms of the final and average displacement errors (FDE and ADE).
However, the multi-modality in these models lacks diversity in the prediction results.
In particular, multi-modal prediction models trained with an imbalanced dataset tend to output multiple trajectories distributed longitudinally, increasing the prediction accuracy in instances of imbalanced validation and test sets even if the outputs are not diverse. (As described in Fig.\ref{figure:1}(a), prediction results are overwhelmed by lane-keeping following the data distribution).
Furthermore, conventional evaluation metrics such as ADE/FDE (Average/Final Displacement Error) encourage these biased results because they only depend on the ground truth in which the majority proceeds straight, and ignoring how diverse the outputs are.
% Furthermore, most conventional works evaluate prediction results based on ADE/FDE(Average/Final Distance Error) metrics, which only depend on the ground truth, thus, can not evaluate diversity at all. 

% which cannot measure the diversity of prediction results quantitatively or qualitatively. 

% Thereby, they can cause critical failure cases by preventing the decision/planning module from proactively taking action with a contingency plan for unexpected futures.

    
    % table for maneuver composition of Argoverse dataset 
    \begin{table}[!t]
    \renewcommand{\arraystretch}{1.4}
    \setlength{\tabcolsep}{12pt}
    \centering
    \caption{Distribution of Target Agents' Maneuver in Argoverse Trajectory Forecasting Dataset } 
    \label{table:data distribution}
    \begin{tabular}{c | c c }
    \hline
    Maneuver & Training  & Validation\\
    \hline
    Going straight & 191024 (92.75\%) & 34958 (90.70\%) \\
    Left turn & 7860 (3.82\%) & 1880 (4.88\%) \\
    Right turn & 4757 (2.31\%) & 1238 (3.21\%) \\
    Left lane change & 1084 (0.53\%) & 284 (0.74\%) \\
    Right lane change & 1217 (0.59\%) & 184 (0.48\%) \\
    \hline
    \end{tabular}
    \vspace{-15pt}
    \end{table}


In this work, we present a method that improves the diversity of multiple-trajectory predictions in a map-adaptive manner. Our novel Lane Loss approach leverages map information to make multiple trajectory outputs cover diverse maneuvers, including those that have never been observed in the ground truth trajectories. 
First, we find multiple feasible reference lanes from the map information and encourage the outputs to be spread over those reference lanes, which can be used as the pseudo GT (Fig.\ref{figure:1}(b)). 
With Lane Loss, the prediction model can output diverse future trajectories, overcoming the imbalance problem and the limitations of unimodal annotation in trajectory datasets. Thereby, downstream motion planners can reckon with uncertain futures during their planning processes. Moreover, because Lane Loss utilizes map information adaptively, it makes the prediction model generalizable for various road environments. It is important to note that the Lane Loss only works in the training phase, and there is no additional burden in terms of inference.

Furthermore, we propose a two-stage trajectory prediction architecture with Trajectory Proposal Attention (TPA), which generates trajectory candidates inspired by a two-stage object detection framework \cite{fastrcnn, fasterrcnn} that leverages region proposals for more accurate detection results. 
TPA generates trajectory proposals in the middle of the prediction model so that the rest of the network can leverage trajectory proposals to output more accurate final prediction results. TPA not only improves the prediction accuracy but also allows Lane Loss to be applied twice for both trajectory candidates and final predictions to enhance the diversity of the prediction results.

Last but not least, we propose a quantitative evaluation metric, minLaneFDE, that can evaluate both the diversity and feasibility at the same time. Because conventional metrics such as the Average Displacement Error (ADE) and the Final Displacement Error (FDE) only measure errors from the ground truth future trajectory, they are impractical for evaluating the diversity of outputs, especially within an imbalanced dataset. To address this problem, minLaneFDE leverages available map information and measures the minimum error between a set of possible lane candidates (feasible maneuvers) and a set of multiple predicted trajectories.  

To summarize, our main contributions are as follows:

\begin{itemize}
\item We devise a loss function that encourages the multiple outputs to be diverse and feasible considering maneuver candidates based on the map information.
\item A two-stage prediction architecture is proposed, which generates trajectory candidates first and leverages them for the final predictions for accuracy and diversity of multiple predictions.
\item We suggest a quantitative evaluation metric, minLaneFDE, that assesses the quality of diversity in multiple outputs in a map-adaptive manner.
\end{itemize}

% The remainder of this paper is organized as follows: In section \ref{sec:Section2}, previous works that are closely related to our work are discussed. 
% In section \ref{sec:Section3}, we will give our problem formulation. Then, the proposed method  including Lane loss and Trajectory Proposal Attention is described in Section \ref{sec:Section4}. 
% In Section \ref{sec:Section5} experiment details such as dataset, implementation details, and results are presented. 
% Finally, Section \ref{sec:Section6} provides the conclusions.

